On Optimizing the Communication of Model Parallelism

We study a novel and important communication pattern in large-scale model-parallel deep learning (DL), which we call cross-mesh resharding. This pattern emerges when the two paradigms of model parallelism - intra-operator and inter-operator parallelism - are combined to support large models on large clusters. In cross-mesh resharding, a sharded tensor needs to be sent from a source device mesh to a destination device mesh, on which the tensor may be distributed with the same or different layouts. We formalize this as a many-to-many multicast communication problem, and show that existing approaches either are sub-optimal or do not generalize to different network topologies or tensor layouts, which result from different model architectures and parallelism strategies. We then propose two contributions to address cross-mesh resharding: an efficient broadcast-based communication system, and an "overlapping-friendly" pipeline schedule. On microbenchmarks, our overall system outperforms existing ones by up to 10x across various tensor and mesh layouts. On end-to-end training of two large models, GPT-3 and U-Transformer, we improve throughput by 10% and 50%, respectively.

==> discussion.tex <==
\section{Contributions}

\subsection{Version 1}
\begin{itemize}

\item Improve single cross-mesh resharding task performance
\begin{itemize}
    \item we use broadcast to reduce the size of messages between two meshes in one resharding task; hence the size of all messages for commucanition in end-to-end settings are also reduced.
    \item we develop an algorithm to achieve better load balancing and time sharing in one resharding task; if there no two resharding competing for one NIC, then globally the load balance will be better.
\end{itemize}
\item Improve multiple cross-mesh resharding tasks performance: 
\begin{itemize}
    \item propose new pipeline schedules which allows more overlapping in normal models like GPT-3
    \item discover new overlapping opportunities in heterogeneous models (such as U-NET), and develop an algorithm to overlap their communication.
\end{itemize}
\end{itemize}


\section{Experiments}

\subsection{Microbenchmarks}
% ray, hoplite, blink (mlsys), microsoft CCL
we construct a few cases to study the effectiveness of our proposed approach.
1. experiment setup: 2 - 3 settings, low-bandwidth, one-NIC setting, nvlink vs. cross-node setting;
2. construct cases: 
3. what to prove: 
\begin{itemize}
    \item broadcast can reduce message sizes on your constructed cases
    \item load balance algorithms can achieve better load balance: (1) load (2) temporal
    % \item new pipeline schedule gives more opportunies ,
    \item we can prove schedule also works via the pipeline bubble graphs
\end{itemize}
4. figure out baselines


\subsection{End-to-end Examples}
Models: GPT-3, u-NET;

Spec: model spec is adjustable in a range.

Baselines: Alpa/Megatron-LM, heurstic algorithms, your method (all optmizations turned on)

Expected results: observe 20\% improvement on end-to-end throughput 

\subsection{Ablation Studies}
1. full optimizations turned on
2. 

\subsection{Microbenchmarks proposed experiments setup}

\subsubsection{reduce message sizes}

    \textbf{One n-to-m send task}
    
    1. experiment setup: I could choose arbitrary instances to show that broadcast could reduce the message size. 
    I am not sure about the effect of multiple NICs. I prefer to only have one NIC in this experiment setup to allow us to focus on reducing the message size. Actually I do not know exactly nccl performs in different intra-node and inter-node topology. But I think I do not need to worry about the effectiveness of nvlink and infiniband. 

    2. construct cases: This is easy. I will have two stages and use two hosts for each stage to show the effectiveness of broadcast. Even in the case that each stage has only one host, broadcast could have few incontiguous data slices and thus give better performance. 
    
    3. what to prove: It is easy to show that broadcast could achieve better result on some cases. But how could I show by experiments that broadcast could achieve better result on all cases? 

    4. baseline: (1) pure send/recv. (2) send/recv+local allgather. 




    \textbf{One resharding task}
    
    Do the same thing as the ``One n-to-m send task''. 

\begin{table*}[]
\begin{tabular}{|p{5cm}|p{3.5cm}|p{7cm}|p{1cm}|}
\hline
{what to prove} &
{experiment} &
{remark} &
{question} \\ \hline
{For a whole resharding task, broadcast is also much faster, given that send/recv have no optimization for load balance and order.} &
{test\_broadcast\_no\_order1; test\_broadcast\_no\_order2;} &
{For these two cases, if we optimize load balance and order, send/recv+allgather could achieve same speed as broadcast. Because load balance could allow multiple send/recv tasks to run in parallel.} &
{} \\ \hline
For a whole resharding task, broadcast is also much faster, no matter using which load balance and order. &
  test\_broadcast\_no\_order3 &
  Besides, I think the above three cases are normal cases &
   \\ \hline
{Even for the case that there is only one dst host, equal cross mesh communication volumn, broadcast is 5\% faster than local allgather} &
{test\_hack\_allgather} &
{} &
{} \\ \hline
\end{tabular}
\end{table*}

    \textbf{Other questions?}
    
    \begin{itemize}
        \item Should I run experiments on multiple data size: 1MB, 32MB, 1G? 
        
        \item Should I run experiments on different number of gpus: 1 gpu/host, 2 gpu/host, 4 gpu/host? 
        \hao{no need to do 1 gpu/host}
        
        \item should I run 10 times and take the average?  \hao{3 warmup + 10 iterations, compute the avg and std}
        \item should I run "n-to-m send task" by broadcast on 1,2,3,...8 hosts to show that broadcast has merely 1\% edge cost for more hosts. (we never use 8 hosts for one stage, honestly. But this could be an edge case).        
    \end{itemize}


\subsubsection{load balance}
    
    \hao{Let's produce results on 1 NICs; multiple NICs experiments can be done later.}
    
    
    \textbf{to show the effectiveness of load balance}
    
    1. experiment setup: I could use one host with multiple NIC to show multiple devices could send data simultaneously using multiple NIC. one host for each stage is enough. I could also use two hosts for one stage and use replicated shardingspec. As long as I could let two devices to send data simultaneously. (May be I could let the device near one NIC to send data.)
    
    2. construct case: simple. 
    
    3. what to prove: load balance could reduce the conjestion at the output of single device. 
    
    4. Baseline: only let one device to send data. 

    
    \textbf{to show the effectiveness of temporal load balance}

    1. experiment setup: (1) If we want to do experiments on a single host-all stages are on the same host. I might need to enumerate types of instances to find the one that could speed up most with load balancing. I think p2p nvswitch(p4d.24xlarge) could help. 
    (2)One host has 4 gpu. we use two stage and each stage has 2 hosts. 
    (3)One host has 1 gpu. we use many hosts. (This is a weird case.) 
    (4)If one host has many nic, then 2 host(1 for send, 1 for recv) should be enough for me to show its effectiveness. However, I need to know its topology in advance to design better strategy. 

    2. construct case: data parallel to model parallel. 
    
    3. what to prove: optimization of the order to send data slice could improve overall performance. I think I could only prove its effectiveness with specified topology. I mean I will describe the topology of my experiment platform in paper. 
    
    4. baseline: has only load balancing over size(let the one with minimal load to send first) but without best sending order. Worse order time and average order time. 

